HTRON:Efficient Outdoor Navigation with Sparse Rewards via Heavy Tailed Adaptive Reinforce Algorithm

We present a novel approach to improve the performance of deep reinforcement learning (DRL) based outdoor robot navigation systems. Most, existing DRL methods are based on carefully designed dense reward functions that learn the efficient behavior in an environment. We circumvent this issue by working only with sparse rewards (which are easy to design), and propose a novel adaptive Heavy-Tailed Reinforce algorithm for Outdoor Navigation called HTRON. Our main idea is to utilize heavy-tailed policy parametrizations which implicitly induce exploration in sparse reward settings. We evaluate the performance of HTRON against Reinforce, PPO and TRPO algorithms in three different outdoor scenarios: goal-reaching, obstacle avoidance, and uneven terrain navigation. We observe in average an increase of 34.41% in terms of success rate, a 15.15% decrease in the average time steps taken to reach the goal, and a 24.9% decrease in the elevation cost compared to the navigation policies obtained by the other methods. Further, we demonstrate that our algorithm can be transferred directly into a Clearpath Husky robot to perform outdoor terrain navigation in real-world scenarios.

==> realted_work_full.tex <==
\section{Related Work}
\label{section:related_work}

\invis{In this section, we discuss existing work on outdoor robot navigation and strategies to address the sparse reward problem.} 

Learning-based approaches, in particular DRL have pushed the boundaries of mobile robot navigation for unstructured and dynamically changing environments~\cite{sathyamoorthy2022terrapn,weerakoon2021terp,liang2022adaptiveon}. Nevertheless these methods suffer form sample efficiency under sparse rewards settings because dense rewards play an important role in learning for DRL methods. We summarize the related work next.  

\textbf{Outdoor Robot Navigation:} Navigation, path planning, and obstacle avoidance are extensively-studied fundamental research problems in the field of robotics \cite{planning_review,motion_planning_survey}. Especially because mobile robots need to autonomously find optimal trajectories (goal‐oriented, and collision‐free) in real‐time to perform successful navigation tasks in both indoor and outdoor environments \cite{mohanan2018survey}. To this end, numerous deterministic \cite{dijkstra1959note,fox1997dwa} and stochastic\cite{kuffner2000rrt,kavraki1996probabilistic} algorithms have been proposed in the past three decades. However, robot navigation in complex outdoor environments still remains a challenging problem given the complexity and diversity of the setting.  Classical approaches used in outdoor robot navigation utilize techniques such as feature classification \cite{pan2020feature_classification}, semantic segmentation \cite{guan2021ganav}, and potential fields \cite{chiang2015potential_fields} to represent terrain traversability. However, such methods are significantly biased towards human annotation \cite{wigness2019rugd}. 
%
To perform a robot-centric decision-making, deep reinforcement learning (DRL) strategies have been employed in recent studies for outdoor navigation \cite{zhou2021review,shah2021ving}. For example, in \cite{josef2020deep_dqn_rainbow}, a DQN network with rainbow architecture is proposed to locally navigate a robot on simulated rough terrains using zero-range to local range elevation sensing. An A3C architecture based DRL network is utilized in \cite{zhang2018uneven_a3c} to determine optimal actions for robot navigation in simulated uneven terrains. Method proposed in \cite{weerakoon2021terp} uses DDPG to train an end-to end DRL network with attention to extract intermediate elevation features for navigation costmap generation. Segmentation methods for identifying navigable regions have also been applied \cite{guan2021ganav},  with combination of DRL based navigation methods ensures stable and efficient navigation. On the other hand the surface properties are possible to learn through self-supervised methods~\cite{sathyamoorthy2022terrapn}. To address the limitation of the predefined characteristics of the traversability of a region that is associated with the specific type of robot, an adaptive model that directly learns control has been studied as well~\cite{liang2022adaptiveon}.

% \ncomment{Can someone put references here from the heavy tailed policy paper lit review?}

\textbf{Sparse Reward Settings:} In sparse reward settings, an environment rarely produces a useful reward which significantly affects the reinforcement policy leaning \cite{zai2020sparse_reward_definition}. To deal with this issue,  several reward shaping methods based on intrinsic curiosity and information gain-based shaping have been proposed in the literature \cite{hussein2017reward_shaping}. For example, reward shaping based methods such as \cite{botteghi2020reward_shaping,houthooft2016vime_reward_shaping} encourage the agent to explore unvisited states by modifying the actual reward output.  However, such approaches require additional effort and expertise in reward function design. Imitation learning and learning from demonstration methods have also been proposed to deal with sparse availability of rewards in practice. For example,in methods \cite{nair2018overcoming_demonstrations}, rewards corresponding to an expert's actions are extracted using inverse reinforcement learning based imitation learning techniques. Learning from expert demonstrations with replay buffers are also employed to improve the policy convergence. However, obtaining reliable expert demonstrations for continuous control tasks is practically infeasible and challenging \cite{ravichandar2020recent,vecerik2017leveraging_sparse_reward}.
%

\textbf{Heavy-tailed Policy Parametrization:} The possibility of incorporating heavy-tailed distributions to RL tasks is theoretically analyzed in recent literature \cite{bedi2021sample_heavy_tailed}. For example, in \cite{chou2017beta}, beta distribution is utilized with dense rewards for stochastic policy training to enhance the state exploration capabilities. Further, a heavy-tailed policy gradient method is proposed in \cite{bedi2021sample_heavy_tailed} to find convergence to global maxima while minimizing the risk of local maxima convergence. Inspired by these ideas, we propose a heavy-tailed adaptive reinforce algorithm to deal with sparse rewards in the complex outdoor environments.

==> tmp.tex <==
% Autonomous robot navigation in complex outdoor environments has drawn a huge attention from the researchers with the increasing emergence of industrial applications such as delivery\cite{delivery}, search and rescue\cite{search_rescue}, agricultural services\cite{agriculture}, planetary explorations\cite{planetary_exploration} etc. Especially, reinforcement learning (RL) techniques have been widely employed in recent robotic systems for navigation\cite{drl_navigation,weerakoon2021terp}. However, efficient Outdoor robotic navigation with continuous control is a hard problem especially for the complexity arising due to the sparse, infrequent and discontinuous rewards\cite{sparse_reward_problem}. Manually crafted and designed dense rewards although can help the robot to navigate and learn with more ease but that is expensive, time-consuming and difficult sometimes. However, a more practical and common form of reward is to use sparse and discontinuous rewards by rewarding the agent at only places while navigating which are critical or after covering a significant, avoiding an obstacle or elevation, reaching a goal etc. Moreover the complexity is significantly higher in continuous control environments like navigation because it’s hard to compute expectations with respect to continuous state and actions distributions for computing the value functions. 

% RL algorithms generally collect rewards and attempt to maximize the expected discounted reward obtain by the agent. 
% Oftentimes, the complex outdoor environment settings lead to reward functions that are quite sparse and designing dense rewards is non-trivial \cite{sparse_reward_problem}. Especially,  designing dense reward functions require a significant effort and expertise on the environment and perception systems. In contrast, sparse rewards are less complex to design and straightforward. However, learning a policy under sparse reward setting is significantly challenging due to \kasun{ mention challenges in learning with sparse rewards}

Autonomous robot navigation in complex outdoor environments finds applications in delivery~\cite{delivery}, search and rescue~\cite{search_rescue}, agricultural services~\cite{agriculture}, and planetary explorations~\cite{planetary_exploration} etc. 
\invis{GIVE A BRIEF OVERVIEW OF WHY AND HOW RL METHODS ARE USED FOR NAVIGATINO (1-2 SENTENCECES)
Deep Reinforcement Learning (DRL) techniques have been widely employed in recent robotic systems for navigation due to ~\cite{drl_navigation,weerakoon2021terp}GIVE MORE REFERENCES TO THESE DRL PAPER.}
%
To generate intelligent navigation decisions in such applications, we require the robots to gather useful information efficiently from the environment  \cite{dhiman2018critical_DRL} and behave accordingly. To this end, Deep Reinforcement Learning (DRL) techniques have been widely deployed in recent robotic systems due to their inherent exploration and exploitation capabilities to gather necessary information over the course of training and then learn suitable policies for the navigation task \cite{drl_navigation,li2019drl_exploration,liang2022adaptiveon}.
%
However, efficient outdoor navigation of mobile robots with continuous state and action spaces control \ncomment{(real valued actions)} space \invis{\dcomment{DEFINE THIS CONCEPT OF CONTINUOUS CONTROL}}is a non-trivial problem, especially with the complexity arising from the sparse, infrequent, and discontinuous rewards~\cite{sparse_reward_problem}. \dcomment{YOU SUDDENTLY INTRODUCE THESE TERMS CORRESPONDING TO SPARSE, INFREQUENT AND DISCONTINUOUS REWARDS. YOU NEED TO DEFINE AND GIVE A BIT MORE CONTEXT} \invis{Moreover, the complexity COMPLEXITY OF WHAT is significantly higher in continuous control environments such as navigation because it’s}For such applications it is a major challenge to estimate expectations with respect to the continuous state and action distributions for value function computations.\cite{bedi2021sample_heavy_tailed} To this end, manually crafted and designed dense rewards are utilized in the literature for policy training. However, designing such dense reward functions  WHAT ARE SOME OF CHARACTERISTICS OF THESE MANUALLY CRAFTED REWARD FUCTIONS> requires a significant effort and expertise in a specific environment and perception systems\cite{bruce2018learning}. As such, a more pragmatic approach is to use sparse and discontinuous rewards by rewarding the agent only during critical instances such as goal-reaching, obstacle avoidance, steep elevations, etc \cite{hare2019dealing_sparse_reward}.

% Outdoor navigation task under challenging environmental configurations including obstacles, uneven terrain, altitude variation with sparse and discontinuous rewards is an extremely critical yet novel problem and there has not been significant research in solving the above problem. In complex navigation problem, the issue has been primarily handled by using reward shaping based methods or demonstration guided learning. The primary objective of rewards shaping based methods revolves inducing the aspect of exploration to learning using various curiosity driven and information theoretic methods. However, such methods require carefully designing the intrinsic rewards which is non-trivial and might end up inducing expert-specific bias to the learning systems hindering the overall performance. The second line of work relies on the expert demonstration or imitation data to provide an initial guidance to the navigation task. The task has shown to perform well in few domains, but the method has extremely high dependence on the presence of expert supervision which again is a big assumption. Moreover, there is a line of work that leverages demonstration in dense navigation tasks, however the availability of such information also seems not practical. 

Outdoor navigation using sparse and discontinuous rewards under challenging environmental configurations such as obstacles, uneven terrains, and altitude variations is an extremely critical problem and there has not been significant research on solving it. In the literature, this issue has been primarily handled by utilizing reward shaping methods\cite{chiang2019learning_reward_shaping} or demonstration-guided learning\cite{vecerik2017leveraging_sparse_reward}. The primary objective of rewards shaping-based methods revolves inducing the aspect of exploration to learn using various curiosity-driven and information-theoretic methods. However, such methods require carefully designed intrinsic rewards which are non-trivial and might end up inducing expert-specific bias to the learning systems hindering the overall performance. The second line of work relies on expert demonstration or imitation learning\cite{karnan2021voila} to provide initial guidance to the navigation task. These strategies have shown improved performance in several domains. However, they have an extremely high dependence on expert supervision which is practically infeasible for many outdoor navigation tasks.

Deterministic policies such as DDPG\cite{weerakoon2021terp}, A3C\cite{zhang2018uneven_a3c}, and DQN\cite{josef2020deep_dqn_rainbow}  with dense rewards have been incorporated in recent literature for outdoor navigation. These methods incorporate high dimensional data from elevation maps, depth images, point cloud, robot's orientation, IMU, etc to define the state space. However, training navigation policies for such high-dimensional state spaces require careful designs of dense reward functions and network architectures. Oftentimes, these methods can consume millions of time steps to converge to an optimal policy which is computationally expensive. 

Sparse rewards can significantly reduce the convergence time in a sample efficient manner. However, we observe that the most common and popular algorithms such as PPO\cite{ppo} and TRPO\cite{trpo} fail to achieve reasonable performance in terms of both average cumulative rewards and robot navigation behavior with sparse reward settings. Although theoretical analysis such as \cite{garg2021proximal} has been conducted in literature to explain the issues in PPO's performance, explicit comparisons and analysis are lacking to understand why the constrained policy gradient methods like PPO and TRPO under perform in sparse reward settings.

Motivate by these factors, in this work, we propose HTRON, a heavy-tailed policy formulation with adaptive tracking and a set of sparse rewards to address three navigation challenges encountered in complex outdoor environments. WHY DO YOU CHOOSE TO USE SUCH AN HEAVY-TAILED POLICY FORMULATION, AND WHAT ARE ITS BENEFITS We summarize the main contributions of our work as follows.

\textbf{Main Contributions:}
\begin{itemize}
    \item We propose a set of novel sparse reward functions that can be utilized to successfully navigate a differential drive robot using an improved stochastic policy gradient method. Sparsity of these reward functions is analyzed using reward surface plots as done in \cite{sullivan2022reward_plots}. WHAT ARE SOME FORMAL METRICS TO EVALUATE THE BENEFITS
    \item  We implement a heavy-tailed policy formulation with adaptive tracking to address three navigation challenges encountered in complex outdoor environments (goal-reaching, obstacle avoidance, and navigating on uneven terrains). Our heavy-tailed policy formulation is inspired by the theoretical analysis presented in  \cite{sparse_reward_souradip} %\kasun{(IROS paper, ICML paper?)}. 
    \item We evaluate our algorithm's performance in both simulated and real-world complex outdoor environments using a Clearpath Husky robot. Our method outperforms three state-of-the-art algorithms Reinforce, PPO and TRPO in terms of both navigation behavior WHAT METRICS OR CHARACTERISTICS ARE USED FOR NAVIGATION BEHAVIOR? GIVE SOME NUMERIC VALUES. and cumulative reward return.
\end{itemize}



% Hence, in this work we focus on generating various complex, discontinuous but practical sparse reward scenarios for outdoor navigation problems including distant goal, multiple obstacles, uneven terrain, altitude variation etc and solve using heavy tailed policy parametrization with adaptive tracking motivated by the theoretical analysis of (our paper). We observe that the most common and popular algorithms like PPO\cite{ppo} and TRPO\cite{trpo} fail to achieve good performance in terms of average cumulative rewards and the robot reaching the goal whereas adaptive heavy tailed reinforce was able to achieve very good rewards and the robot reached the goal in various settings. Although, there have been theoretical analysis done in (cite cmu's paper) to explain the issues in PPO's performance, but there has not been done explicit comparisons and analysis why constrained policy gradient methods like PPO and TRPO underperform in Sparse navigation tasks. We also analyze the reason with reward curvature based analysis as done in (cite Ryan's paper) which gives us a very good intuition on the improvement in performance of such heavy tailed parametrizations. 

The rest of this paper is organized as follows. First, an overview of related work is presented in Section~\ref{section:related_work}. In Section~\ref{section:proposed_method}, we give an overview of the fundamental mathematical models that this work is base of and proceed with a formal definition of the problem along with details of the proposed approach. We report the experimental results in Section~\ref{section:experiments} for three different scenarios based on their complexity. Finally we discuss the limitations of our work in Section~\ref{section:limitations} and draw conclusions are in Section~\ref{section:conclusion}. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth,height=7cm]{figures/cat.jpg}
%     \caption{Cover Image}
%     \label{fig:cover-imagel}
% \end{figure}



